Subsets of Rectifiable curves in Hilbert Space-The Analyst's TSP

We study one dimensional sets (Hausdorff dimension) lying in a Hilbert space. The aim is to classify subsets of Hilbert spaces that are contained in a connected set of finite Hausdorff length. We do so by extending and improving results of Peter Jones and Kate Okikiolu for sets in $\R^d$. Their results formed the basis of quantitative rectifiability in $\R^d$. We prove a quantitative version of the following statement: a connected set of finite Hausdorff length (or a subset of one), is characterized by the fact that inside balls at most scales around most points of the set, the set lies close to a straight line segment (which depends on the ball). This is done via a quantity, similar to the one introduced in \cite{Jones90}, which is a geometric analog of the Square function. This allows us to conclude that for a given set $K$, the $\ell_2$ norm of this quantity (which is a function of $K$) has size comparable to a shortest (Hausdorff length) connected set containing $K$. In particular, our results imply that, with a correct reformulation of the theorems, the estimates in \cite{Jones90,Okik92} are {\bf independent of the ambient dimension}.

==> pics/new_weight_example_nh.tex <==
\begin{figure}[p]
\begin{center}
$\begin{array}{c@{\hspace{.2in}}c}
%
\scalebox{0.25}{\includegraphics*[0in,0in][8.5in,8in]{pics/new_weight_00.eps}}&
\scalebox{0.25}{\includegraphics*[0in,0in][8.5in,8in]{pics/new_weight_0.eps}}\\
\mbox{Several  crossing segments.} & \mbox{With $U_{Q}$'s.}\\
&\mbox{We have $M=1$.}\\
&\mbox{We assume these are the only $U_Q$'s.}\\[0.4cm]
% \end{array}$
%%
%$\begin{array}{c@{\hspace{0.2in}}c}
\scalebox{0.25}{\includegraphics*[0in,0in][8.5in,8in]{pics/new_weight_1.eps}}&
   \scalebox{0.25}{\includegraphics*[0in,0in][8.5in,8in]{pics/new_weight_2.eps}}\\
U_{Q_1}&U_{Q_2}\\
 \end{array}$
\end{center}
\caption{An  example of weight distribution arising form the martingale. Second example}
\label{new_weight}
\end{figure}



